Training Larger Networks for Deep Reinforcement Learning

The success of deep learning in the computer vision and natural language processing communities can be attributed to training of very deep neural networks with millions or billions of parameters which can then be trained with massive amounts of data. However, similar trend has largely eluded training of deep reinforcement learning (RL) algorithms where larger networks do not lead to performance improvement. Previous work has shown that this is mostly due to instability during training of deep RL agents when using larger networks. In this paper, we make an attempt to understand and address training of larger networks for deep RL. We first show that naively increasing network capacity does not improve performance. Then, we propose a novel method that consists of 1) wider networks with DenseNet connection, 2) decoupling representation learning from training of RL, 3) a distributed training method to mitigate overfitting problems. Using this three-fold technique, we show that we can train very large networks that result in significant performance gains. We present several ablation studies to demonstrate the efficacy of the proposed method and some intuitive understanding of the reasons for performance gain. We show that our proposed method outperforms other baseline algorithms on several challenging locomotion tasks.

==> background_old.tex <==
\section{Background}
In this section, we provide relevant background that are used throughout the paper.
We first describe the off-policy actor-critic framework, which will be a basic framework for our approach.
Then, we explain a specific SRL method that can provide higher dimensional representation.
Next, we explain a distributed RL framework and network architecture.
Finally, we show a recently introduced metric to evaluate the performance of a neural network.

% \subsection{Off-policy actor-critic}
% We consider a standard RL setup with the actor-critic method as an agent, where the actor $\pi_\phi(a | s)$ and the critic $Q_\theta(s, a)$ are both parameterized by neural networks.
% Specifically, we consider the \emph{off-policy} methods that allows us to use transitions collected by different policies from the current one, thus improves sample efficiency~\cite{watkins1992qlearning}.
% In the experiments, we use proposed soft actor critic (SAC)~\cite{haarnoja2018soft}.
% % twin delayed deep deterministic policy gradient algorithm(TD3)~\cite{fujimoto2018addressing} and 
% % \konote{Here we explicitly state that our method focuses on off-policy actor-critic method, such as TD3 and SAC.}

\subsection{Online Feature Extractor Network} \label{sec:background_ofenet}
In order to learn larger networks, it would be ideal to obtain a good signal to be used for train a part of the large network.
\cite{ota2020can} recently proposed the online feature extractor network (OFENet), which learns representation vectors of states and state-action pairs, and provides them to the agent instead of original inputs, giving significant performance improvements on continuous robot control tasks.
The state representation $z_{s_t}$ and state-action representation $z_{s_t,a_t}$.
The representations can be obtained by learning the mappings $z_{s_t}=\phi_s(s_t)$ and $z_{s_t,a_t}=\phi_{s,a}(s_t,a_t)$, which have parameters $\theta_{\phi_s}, \theta_{\phi_{s,a}}$.
In order to learn the mappings, it uses an auxiliary task whose goal is to predict the next state $s_{t+1}$ from the current state and action.
The learning of the auxiliary task is done concurrently with the learning of the downstream RL task.

\subsection{Distributed Reinforcement Learning}
Distributed RL has achieved significant improvement by leveraging distributed training architectures which decouples learning from collecting transitions by utilizing many actors running in parallel on separate environment instances~\cite{horgan2018distributed,kapturowski2018recurrent}.

Ape-X~\cite{horgan2018distributed} has a distributed replay where many actors collect data with priorities and a learner receives training batches from the prioritized replay buffer. It showed state-of-the-art results both on discrete and continuous control domains.

\subsection{Network Architectures}\label{sec:background_architectures}
The CNNs used by the computer vision community have been growing deeper and deeper since \citet{krizhevsky2012imagenet} proposed AlexNet in 2012.
In order to train such deep networks, many recent publications address an efficient network architectures.
% the vanishing gradient problem: the gradient can vanish as it passes through many layers.

Residual networks (ResNet)~\cite{he2016deep,he2016identity} adds a skip-connection that bypasses the non-linear transformations with an identity function: $y_{i} = f_i^\text{res}(y_{i-1}) + y_{i-1}$, where $y_i$ is the output of the $i^{th}$ layer, and $f_i^\text{res}$ is a residual module.
An advantage of this architecture is that the gradient can flow directly through the identity mapping from top layers to bottom layers.
Commonly in computer vision community, the residual module $f_i^\text{res}$ consists of some sequence of convolutions, batch normalization~\cite{ioffe2015batch}, and Rectified Linear Units (ReLU) as activation function.

Dense Convolutional Network (DenseNet)~\cite{huang2017densely} proposes a different skip connection pattern: it directly connects each layer to all subsequent layers as: $y_{i} = f_i^\text{dense}([ y_0, y_1, ..., y_{i-1}])$ in which all the inputs are concatenated into a single tensor, and $f_i^\text{dense}$ is a composite function similar to $f_i^\text{res}$.
An advantage of DenseNets is their improved flow of information and grdients throughout the network, which makes them easy to train. Each layer has direct access to the gradients from the loss function and the original input signal, which helps training of deeper network architectures.
% It ensures maximum information flow between layers in the network as all of them are directly connected with each other.
% It alleviates the vanishing-gradient problem, strengthen feature propagation,
% encourage feature reuse, and substantially reduce the number of parameters.

In DRL comminity, \cite{sinha2020d2rl} proposes D2RL, which is a DenseNet-like architecture, and used for both the policy and value function networks to train deeper networks.
D2RL concatenates the state or the state-action pair to each hidden layer of the networks except the last output linear layer.
OFENet~\cite{ota2020can} uses MLP-DenseNet, which is a modified version of DenseNet for MLP for state representation learning, and demonstrates it helps improve the performance of downstream RL tasks. They also compare performance against MLP and MLP-ResNet, and showed MLP-DenseNet is the best architecture to generate good features. It is noted that OFENet uses the MLP-DenseNet only for state representation learning, nor RL.

\subsection{Implicit under-parameterization}
\citet{kumar2021implicit} characterize implicit under-parameterization in terms of the \emph{effective rank} of the features $\text{srank}_\delta(\Phi)$ learned by a Q-network. It shows both theoretically and empirically that the lower the rank, the poorer the performance of RL agents.
% While the performance of RL agents cannot measure with this single metric, we believe this is a good metric considering the ...
We believe that our combination of feature learning, network architecture, and distributed training can help alleviate the rank collapse issue, and thus employ this metric to evaluate the validity of our proposed architecture.


==> method_old.tex <==
\section{Method} \label{sec:methods}
While recent study suggests that larger networks for DRL agents have potential to improve performance, we also need to resolve some potential issues that occur when increasing network capacity.
This section describes our method that aims to improve performance by overcoming those problems.

Our method consists of three elements: 1) decoupling representation learning and RL, 2) distributed learning, and 3) employing DenseNet architecture.
In this section, we describe these components in detail.

\begin{figure*}
    \centering
    \includegraphics[width=0.8\textwidth]{fig/architecture.png}
    \caption{Proposed architecture.}
    \label{fig:architecture}
\end{figure*}

\subsection{Decoupling Representation Learning from RL}
While the simplicity of learning whole networks in end-to-end fashion is appealing, updating all parameters of a large network from just a scalar reward signal can result in very data inefficient~\cite{stooke2020decoupling}.
Decoupling unsupervised pretraining from downstream tasks is common in computer vision~\cite{he2020momentum,henaff2020data}.
Taking inspiration from this, we also adopt SRL methods to learn meaningful features apart from RL.
Among many SRL methods have been proposed, we choose to use OFENet~\cite{ota2020can} for the following reasons: 1) OFENet allows to obtain informative representations on-line, which does not need expert demonstrations beforehand to build a good representation, 2) it can provide much larger features than inputs, which matches our philosophy that larger solution space can allow us to find better policy, and 3) task-agnostic features allows us to build a general-purpose method since it just predicts next states from current states and actions.

\subsection{Distributed Training}\label{sec:method_dist_sample}
In general, larger networks tend to need more data to improve accuracy of function approximation~\cite{bishop2006pattern}. \konote{cite papers that support MLP can be easier to overfit when being larger.}
A simple workaround to learn such larger networks is just increasing the size of dataset.
In fact, the common dataset CV community uses has grown larger and larger [cite].
\konote{Is this logic easy to understand? We might not need to contrast with CV community?}

In the context of RL, the networks can overfit to data stored in its replay buffer~\cite{fu2019diagnosing,fedus2020revisiting}, which can be considered becomes much worse when we use larger networks.
To mitigate this potential problem, we employ Ape-X~\cite{horgan2018distributed} framework, where a single learner receives data from distributed prioritized replay~\cite{schaul2016prioritized}, and multiple actors collect transitions in parallel.
We expect this can not only mitigate overfitting problem but also improves control performance as the distributed replay can provide more on-policy data, which can improve performance according to~\cite{fedus2020revisiting}.
One difference is that we do not use the RL algorithm used in~\cite{horgan2018distributed}, but instead use standard off-policy RL algorithms: SAC~\cite{haarnoja2018soft} and Twin Delayed Deep Deterministic policy
gradient algorithm (TD3)~\cite{fujimoto2018addressing} in our experiments.

% A simple method to mitigate this potential problem is increasing the number of data to update the agent while applying one gradient step. Distributed RL enables this as it decouples learning and collecting transitions: the separate actors collect transitions on different CPU cores~\cite{horgan2018distributed,kapturowski2018recurrent}.
% We specifically employ Ape-X~\cite{horgan2018distributed} as a distributed RL framework.
% We employ a distributed method to increase the number of samples while one gradient step is applied.
% We expect this mitigates distribution mismatch as it enables the agent to learn from more on-policy data, and thus mitigate overfitting to more off-policy data in replay buffer~\cite{achiam2019towards,fedus2020revisiting}.

% We employ ApeX-like~\cite{horgan2018distributed} sampling with an 
% % , which collects experiences using $M$ cores on which each core contains $N$ environments. Please see~\ref{apppendix:distributed_sampling} for more details.
% \konote{State here that we're using huber loss.}

\subsection{Network Architecture}\label{sec:method_architecture}
In order to train larger networks, we borrow a useful technique originally developed in computer vision community, DenseNet~\cite{huang2017densely}.
DenseNet connects each layer to every other layer, and this enables to alleviate the vanishing-gradient problem, and strengthen feature propagation.
Using the DenseNet architecture for DRL is not new. D2RL~\cite{sinha2020d2rl} employs the modified DenseNet architecture, which concatenates the state or the state-action pair to each hidden layer of the MLP networks except the last output linear layer.
Based on our empirical finding of the performance gain, we use the dense connection similar to the one used in~\cite{ota2020can}, which concatenates the all outputs of the previous layer instead of only the state or the state-action pair done in~\cite{sinha2020d2rl}.

